When to Speak, When to Abstain: Contrastive Decoding with Abstention

Large Language Models (LLMs) demonstrate exceptional performance across diverse tasks by leveraging pre-trained (i.e., parametric) and external (i.e., contextual) knowledge. While substantial efforts have been made to enhance the utilization of both forms of knowledge, situations in which models lack relevant information remain underexplored. To investigate this challenge, we first present a controlled testbed featuring four distinct knowledge access scenarios, including the aforementioned edge case, revealing that conventional LLM usage exhibits insufficient robustness in handling all instances. Addressing this limitation, we propose Contrastive Decoding with Abstention (CDA), a novel training-free decoding method that allows LLMs to generate responses when relevant knowledge is available and to abstain otherwise. CDA estimates the relevance of both knowledge sources for a given input, adaptively deciding which type of information to prioritize and which to exclude. Through extensive experiments, we demonstrate that CDA can effectively perform accurate generation and abstention simultaneously, enhancing reliability and preserving user trust.

==> assets/images/case_study.tex <==

% \begin{figure}[t]
%     \centering
%     \begin{subfigure}{\columnwidth}
%         \includegraphics[width=0.98\columnwidth]{assets/tmp/cda_compare.png} 
%         \caption{CDA vs CDA-m}
%     \end{subfigure}
    
%     \begin{subfigure}{\columnwidth}
%         \includegraphics[width=0.98\columnwidth]{assets/tmp/cda_fixed_compare.png} 
%         \caption{$\alpha$=0 vs $\alpha$=0.7}
%     \end{subfigure}
    

%     \caption{
%         CDA-m에서 momentum weight $\alpha$의 영향을 분석하기 위한 예시.
%         (a) CDA ($\alpha$=0.0) 와 CDA-m ($\alpha$=0.7)의 비교. 
%         새로 생성된 token에 의해 발생하는 잘못된 bias를 momentum을 통해 mitigate할 수 있음.
%         (b) CDA-m 중 $\alpha$=1.0 인 경우와 $\alpha$=0.7인 경우를 비교.
%         $\alpha$=1.0 인 경우는 첫 step에서 결정된 weight로 끝까지 decoding 하는 방식임.
%         현재 step을 반영해야지 시점마다 적절한 knowledge를 반영할 수 있다는 것을 확인할 수 있음.
%         CDA-m은 momentum을 통해 잘못된 bias가 형성되는 것을 방지할 뿐만 아니라, 
%         적절한 시점에 필요한 knowledge를 decoding 과정에 반영하도록 도와줌.
%     }
%     \label{figure:case_study}
% \end{figure}



\begin{figure*}[t]
    \centering
    \begin{subfigure}{0.49\linewidth}
        \includegraphics[width=\linewidth]{assets/tmp/cda_compare.png} 
        \caption{CDA vs CDA-m}
    \end{subfigure}
    \begin{subfigure}{0.49\linewidth}
        \includegraphics[width=\linewidth]{assets/tmp/cda_fixed_compare.png} 
        \caption{$\alpha$=0 vs $\alpha$=0.7}
    \end{subfigure}
    

    \caption{
        CDA-m에서 momentum weight $\alpha$의 영향을 분석하기 위한 예시.
        (a) CDA ($\alpha$=0.0) 와 CDA-m ($\alpha$=0.7)의 비교. 
        새로 생성된 token에 의해 발생하는 잘못된 bias를 momentum을 통해 mitigate할 수 있음.
        (b) CDA-m 중 $\alpha$=1.0 인 경우와 $\alpha$=0.7인 경우를 비교.
        $\alpha$=1.0 인 경우는 첫 step에서 결정된 weight로 끝까지 decoding 하는 방식임.
        현재 step을 반영해야지 시점마다 적절한 knowledge를 반영할 수 있다는 것을 확인할 수 있음.
        CDA-m은 momentum을 통해 잘못된 bias가 형성되는 것을 방지할 뿐만 아니라, 
        적절한 시점에 필요한 knowledge를 decoding 과정에 반영하도록 도와줌.
    }
    \label{figure:case_study}
\end{figure*}

==> assets/images/data_processing.tex <==

\begin{figure*}[t]
    \centering
    
    \includegraphics[width=0.97\linewidth]{assets/tmp/data_processing.pdf}

    \caption{
        Visualization of the controlled analysis setup process.
    }
    \label{figure:data_processing}
\end{figure*}


==> assets/images/intro_figure_old.tex <==


\begin{figure}[t]
    \centering
    
    \includegraphics[width=0.99\linewidth]{assets/tmp/intro.pdf} 

    \caption{
        This study considers two primary scenarios.
        First, when relevant knowledge is present within the model, it is expected to generate a response grounded in that knowledge.
        Second, when no relevant knowledge is available, the model should abstain from producing potentially inaccurate or misleading outputs.
    }
    \label{figure:intro_figure}
\end{figure}

==> assets/images/momentum_ablation.tex <==

\begin{figure}[t]
    \begin{center}
        
    % \begin{subfigure}{\columnwidth}
    %     \includegraphics[width=\textwidth]{assets/tmp/momentum_nq.pdf} 
    %     \caption{NQ}
    % \end{subfigure}
    
    % \begin{subfigure}{\columnwidth}
    %     \includegraphics[width=\textwidth]{assets/tmp/momentum_hotpot_qa.pdf} 
    %     \caption{HotpotQA}
    % \end{subfigure}

    % \begin{subfigure}{\columnwidth}
    %     \includegraphics[width=\textwidth]{assets/tmp/momentum_trivia_qa.pdf} 
    %     \caption{TriviaQA}
    % \end{subfigure}

    
    % \includegraphics[width=0.97\columnwidth]{assets/tmp/alpha_ablation.pdf}
    \includegraphics[width=0.92\columnwidth]{assets/tmp/momentum_ablation.pdf}
        
          \caption{
            % Changes in \ans{} and \abs{} according to $\alpha$.
            \ans{} and \abs{} according to different $\alpha$ values.
            Applying momentum significantly improves \ans{}.
            % \abs{} remains consistent regardless of $\alpha$, but significantly improves \ans{}.
          }
          \label{figure:alpha_ablation}
    \end{center}
\end{figure}

==> assets/images/problem_formulation.tex <==

\begin{figure}[t!]
    \centering
    
    \includegraphics[width=0.97\columnwidth]{assets/tmp/problem_formulation.pdf}

    
    \caption{
        % Four possible scenarios regarding the model's parametric and contextual knowledge.
        % The model is expected to generate factual responses when relevant knowledge is present or else abstain from answering.
        Four possible scenarios according to the existence of the model's parametric and contextual knowledge. 
        The model is expected to generate \textit{reliable} responses based on its possessed knowledge.
        % The model is expected to generate accurate responses when relevant knowledge is present.
        % Otherwise, it should abstain from generating irrelevant responses.
    }
    \label{figure:problem_formulation}
\end{figure}

==> assets/images/radar_chart.tex <==

\begin{figure}[t]
    \begin{center}
        \includegraphics[width=0.57\columnwidth]{assets/tmp/overall_performance_figure.pdf}
          \caption{
            % Average performance across all metrics compared with the strongest baselines (\acd{}, \fsb{})
            Average performance compared with the strongest baselines (\acd{}, \fsb{}).
            The area covered by each method is indicated in parentheses.
            % , with larger areas reflecting its overall effectiveness.
            \methodm{} covers the largest area, indicating superior performance across all metrics.
            % overall performance.
            Individual results are provided in Figure \ref{figure:radar_chart_full}.
            % The results for each scenario are provided in Figure \ref{figure:radar_chart_full}.
          }
          \label{fig:radar_chart}
    \end{center}
\end{figure}

==> assets/images/radar_chart_full.tex <==

\begin{figure*}[t]
    \centering
    \begin{subfigure}{0.31\linewidth}
        \centering
        \includegraphics[width=0.85\linewidth]{assets/tmp/llama2_7_nq.pdf} 
        \caption{\ml{} NQ}
    \end{subfigure}
    \begin{subfigure}{0.31\linewidth}
        \centering
        \includegraphics[width=0.85\linewidth]{assets/tmp/llama2_7_hotpot.pdf} 
        \caption{\ml{} HotpotQA}
    \end{subfigure}
    \begin{subfigure}{0.31\linewidth}
        \centering
        \includegraphics[width=0.85\linewidth]{assets/tmp/llama2_7_trivia.pdf} 
        \caption{\ml{} TriviaQA}
    \end{subfigure}
    
    \begin{subfigure}{0.31\linewidth}
        \centering
        \includegraphics[width=0.85\linewidth]{assets/tmp/llama2_13_nq.pdf} 
        \caption{\mll{} NQ}
    \end{subfigure}
    \begin{subfigure}{0.31\linewidth}
        \centering
        \includegraphics[width=0.85\linewidth]{assets/tmp/llama2_13_hotpot.pdf} 
        \caption{\mll{} HotpotQA}
    \end{subfigure}
    \begin{subfigure}{0.31\linewidth}
        \centering
        \includegraphics[width=0.85\linewidth]{assets/tmp/llama2_13_trivia.pdf} 
        \caption{\mll{} TriviaQA}
    \end{subfigure}
    
    \begin{subfigure}{0.31\linewidth}
        \centering
        \includegraphics[width=0.85\linewidth]{assets/tmp/llama3_nq.pdf} 
        \caption{\mlll{} NQ}
    \end{subfigure}
    \begin{subfigure}{0.31\linewidth}
        \centering
        \includegraphics[width=0.85\linewidth]{assets/tmp/llama3_hotpot.pdf} 
        \caption{\mlll{} HotpotQA}
    \end{subfigure}
    \begin{subfigure}{0.31\linewidth}
        \centering
        \includegraphics[width=0.85\linewidth]{assets/tmp/llama3_trivia.pdf} 
        \caption{\mlll{} TriviaQA}
    \end{subfigure}
    
    \begin{subfigure}{0.31\linewidth}
        \centering
        \includegraphics[width=0.85\linewidth]{assets/tmp/mistral_nq.pdf} 
        \caption{\mm{} NQ}
    \end{subfigure}
    \begin{subfigure}{0.31\linewidth}
        \centering
        \includegraphics[width=0.85\linewidth]{assets/tmp/mistral_hotpot.pdf} 
        \caption{\mm{} HotpotQA}
    \end{subfigure}
    \begin{subfigure}{0.31\linewidth}
        \centering
        \includegraphics[width=0.85\linewidth]{assets/tmp/mistral_trivia.pdf} 
        \caption{\mm{} TriviaQA}
    \end{subfigure}
    

    \caption{
        Individual results for all datasets and backbones compared with the strongest baselines (\acd{}, \fsb{})
            The area covered by each method is indicated in parentheses.
            Overall, \methodm{} covers the largest area, indicating superior performance across all metrics.
    }
    \label{figure:radar_chart_full}
\end{figure*}

==> assets/tables/external_verifier_full.tex <==
\definecolor{bg}{HTML}{b1d4e0}

\begin{table}[t]
    \centering
               
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ccccc}
    \toprule
    Source & Target & \abs{} & \ans{} & RS \\ 
    \midrule
    \multirow{3}{*}{NQ} & 
    \cellcolor{bg}NQ & 
    \cellcolor{bg}64.86 \footnotesize{(1.49)} &
    \cellcolor{bg}46.56 \footnotesize{(3.17)} & 
    \cellcolor{bg}58.03 \footnotesize{(1.06)} \\
     & HotpotQA & 66.62 \footnotesize{(1.90)} & 52.36 \footnotesize{(2.61)} & 58.50 \footnotesize{(1.16)} \\
     & TriviaQA & 65.07 \footnotesize{(2.09)} & 53.52 \footnotesize{(3.07)} & 57.39 \footnotesize{(2.17)} \\ 
    \midrule
    \multirow{3}{*}{HotpotQA} & NQ & 61.46 \footnotesize{(3.13)} & 38.42 \footnotesize{(8.06)} & 54.60 \footnotesize{(2.15)} \\
     & \cellcolor{bg}HotpotQA & 
     \cellcolor{bg}68.41 \footnotesize{(0.22)} & 
     \cellcolor{bg}56.92 \footnotesize{(1.32)} & 
     \cellcolor{bg}60.80 \footnotesize{(1.12)} \\
     & TriviaQA & 60.09 \footnotesize{(2.37)} & 38.53 \footnotesize{(11.96)} & 53.28 \footnotesize{(1.04)} \\ 
    \midrule
    \multirow{3}{*}{TriviaQA} & NQ & 63.30 \footnotesize{(0.74)} & 45.10 \footnotesize{(5.07)} & 55.55 \footnotesize{(0.27)} \\
     & HotpotQA & 66.97 \footnotesize{(0.19)} & 54.88 \footnotesize{(0.98)} & 59.24 \footnotesize{(0.26)} \\
     & \cellcolor{bg}TriviaQA & 
     \cellcolor{bg}65.31 \footnotesize{(1.14)} & 
     \cellcolor{bg}52.63 \footnotesize{(2.56)} & 
     \cellcolor{bg}58.13 \footnotesize{(0.43)} \\ 
     \bottomrule
    \end{tabular}

    
    }
    
    \caption{
        Average and standard deviation (in parentheses) of external verifier over three different random seeds.
        \colorbox{bg}{In-domain} results are highlighted in blue.
    }
    \label{table:external_verifier_full}
\end{table}




==> assets/tables/instruction_tuning_full.tex <==
% \definecolor{bg}{HTML}{b1d4e0}

% \begin{table}[t]
%     \centering
        
%     \begin{subfigure}{0.99\columnwidth}
%         \centering
%         \resizebox{0.8\linewidth}{!}{

%         % begin tabular ~ end tabular goes here
%         \begin{tabular}{ccccc}
%         \toprule
%         Source & Target & \ans{} & \abs{} & RS \\ 
%         \midrule
%         \multirow{5}{*}{NQ} & 
%         \cellcolor{bg}NQ & 
%         \cellcolor{bg} 66.37\\ \footnotesize{(0.55)} &
%         \cellcolor{bg} 43.87\\ \footnotesize{(2.02)} &
%         \cellcolor{bg} 61.12\\ \footnotesize{(0.46)} \\
%          & HotpotQA &  64.43\\ \footnotesize{(0.42)} &  48.79\\ \footnotesize{(3.88)} &  59.65\\ \footnotesize{(0.42)} \\
%          & TriviaQA & 
%           67.31\\ \footnotesize{(1.82)} &
%           49.00\\ \footnotesize{(4.74)} &
%           62.14\\ \footnotesize{(1.43)} \\ 
%          \bottomrule
%         \end{tabular}

%         }
         
%         \caption{Results of instruction-tuning trained on NQ dataset.}
        
%     \end{subfigure}

%     \begin{subfigure}{0.99\columnwidth}
%         \centering
%         \resizebox{0.8\linewidth}{!}{

%         % begin tabular ~ end tabular goes here
%         \begin{tabular}{ccccc}
%         \toprule
%         Source & Target & \ans{} & \abs{} & RS \\ 
%         \midrule
%         \multirow{5}{*}{HotpotQA} & NQ &  64.86\\ \footnotesize{(2.38)} &  4.273\\ \footnotesize{(1.49)} &  59.80\\ \footnotesize{(1.92)} \\
%          & 
%          \cellcolor{bg}HotpotQA & 
%          \cellcolor{bg} 74.06\\ \footnotesize{(0.76)} &
%          \cellcolor{bg} 57.57\\ \footnotesize{(0.73)} &
%          \cellcolor{bg} 68.76\\ \footnotesize{(0.81)} \\
%          & TriviaQA &  65.26\\ \footnotesize{(4.92)} &  50.69\\ \footnotesize{(2.06)} &  61.17\\ \footnotesize{(4.10)} \\ 
%          \bottomrule
%         \end{tabular}

        
%         }
%         \caption{Results of instruction-tuning trained on HotpotQA dataset.}
        
%     \end{subfigure}

    
%     \begin{subfigure}{0.99\columnwidth}
%         \centering
%         \resizebox{0.8\linewidth}{!}{

%         % begin tabular ~ end tabular goes here
%         \begin{tabular}{ccccc}
%         \toprule
%         Source & Target & \ans{} & \abs{} & RS \\ 
%         \midrule
%         \multirow{5}{*}{TriviaQA} & NQ &  65.15\\ \footnotesize{(1.66)} &  46.37\\ \footnotesize{(4.00)} &  59.70\\ \footnotesize{(1.10)} \\
%          & HotpotQA &  66.68\\ \footnotesize{(0.13)} &  49.82\\ \footnotesize{(3.52)} &  60.58\\ \footnotesize{(0.25)} \\
%          & 
%          \cellcolor{bg}TriviaQA &
%          \cellcolor{bg} 67.60\\ \footnotesize{(1.73)} &
%          \cellcolor{bg} 53.68\\ \footnotesize{(2.92)} &
%          \cellcolor{bg} 61.84\\ \footnotesize{(0.70)} \\ 
%          \bottomrule
%         \end{tabular}

        
%         }
%         \caption{Results of instruction-tuning trained on TriviaQA dataset.}
        
%     \end{subfigure}
    
%     \caption{
%         The results of the trained methods and \methodm{}.
%         \colorbox{bg}{In-domain} results are highlighted in blue and the \textbf{best results} are in bold.
%         \methodm{} outperforms the trained methods across all the scenarios.
%     }
%     \label{table:trained_methods_v2}
% \end{table}




\definecolor{bg}{HTML}{b1d4e0}

\begin{table}[t]
    \centering

    \resizebox{0.99\linewidth}{!}{

        % begin tabular ~ end tabular goes here
        \begin{tabular}{ccccc}
        \toprule
        Source & Target & \ans{} & \abs{} & RS \\ 
        \midrule
        \multirow{3}{*}{NQ} & 
        \cellcolor{bg}NQ & 
        \cellcolor{bg} 66.37 \footnotesize{(0.55)} &
        \cellcolor{bg} 43.87 \footnotesize{(2.02)} &
        \cellcolor{bg} 61.12 \footnotesize{(0.46)} \\
         & HotpotQA &  
         64.43 \footnotesize{(0.42)} &  
         48.79 \footnotesize{(3.88)} &
         59.65 \footnotesize{(0.42)} \\
         & TriviaQA & 
          67.31 \footnotesize{(1.82)} &
          49.00 \footnotesize{(4.74)} &
          62.14 \footnotesize{(1.43)} \\ 
         \midrule
         
        \multirow{3}{*}{HotpotQA} & 
        NQ &  
        64.86 \footnotesize{(2.38)} &
        42.73 \footnotesize{(1.49)} &  
        59.80 \footnotesize{(1.92)} \\
         & 
         \cellcolor{bg}HotpotQA & 
         \cellcolor{bg} 74.06 \footnotesize{(0.76)} &
         \cellcolor{bg} 57.57 \footnotesize{(0.73)} &
         \cellcolor{bg} 68.76 \footnotesize{(0.81)} \\
         & TriviaQA &  
         65.26 \footnotesize{(4.92)} &
         50.69 \footnotesize{(2.06)} &
         61.17 \footnotesize{(4.10)} \\ 
         
        \midrule
        \multirow{3}{*}{TriviaQA} & 
        NQ &  
        65.15 \footnotesize{(1.66)} &
        46.37 \footnotesize{(4.00)} &
        59.70 \footnotesize{(1.10)} \\
         & HotpotQA &  
         66.68 \footnotesize{(0.13)} &
         49.82 \footnotesize{(3.52)} &
         60.58 \footnotesize{(0.25)} \\
         & 
         \cellcolor{bg}TriviaQA &
         \cellcolor{bg} 67.60 \footnotesize{(1.73)} &
         \cellcolor{bg} 53.68 \footnotesize{(2.92)} &
         \cellcolor{bg} 61.84 \footnotesize{(0.70)} \\ 
         \bottomrule
        \end{tabular}

        
        }
            
    \caption{
        Average and standard deviation (in parentheses) of instruction-tuning over three different random seeds.
        \colorbox{bg}{In-domain} results are highlighted in blue.
    }
    \label{table:instruction_tuning_full}
\end{table}




==> assets/tables/main_results.tex <==
\definecolor{my_gray}{HTML}{E8E8E8}
\newcolumntype{g}{>{\columncolor{my_gray}}c}



\begin{table*}[t!]
    \centering    
    \resizebox{0.83\textwidth}{!}{

  \begin{tabular}{ccgggcccgggccc}
\toprule

\multicolumn{2}{c}{Backbone} &
\multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}} {\scshape Llama3 8B}\\ {\scshape Instruct}\end{tabular}} &
\multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}} {\scshape Llama2 7B}\\ {\scshape Chat}\end{tabular}} &
\multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}} {\scshape Llama2 13B}\\ {\scshape Chat}\end{tabular}} &
\multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}} {\scshape Mistral 7B}\\ {\scshape Instruct}\end{tabular}} \\
\midrule
% \cmidrule(l){1-2} \cmidrule(l){3-5} \cmidrule(l){6-8} \cmidrule(l){9-11} \cmidrule(l){12-14} 
Dataset & Method & \multicolumn{1}{c}{\ans{}} & \multicolumn{1}{c}{\abs{}} & \multicolumn{1}{c}{RS} &
\multicolumn{1}{c}{\ans{}} & \multicolumn{1}{c}{\abs{}} & \multicolumn{1}{c}{RS} &
\multicolumn{1}{c}{\ans{}} & \multicolumn{1}{c}{\abs{}} & \multicolumn{1}{c}{RS} &
\multicolumn{1}{c}{\ans{}} & \multicolumn{1}{c}{\abs{}} & \multicolumn{1}{c}{RS} \\ 
\midrule
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multirow{10}{*}{NQ} & 
\context{} & 57.26 & 2.18 & 50.22 & 57.13 & 0.09 & 49.98 & 57.14 & 0.37 & 50.00 & 57.04 & 0.25 & 49.88 \\
 & \cad{} & 55.34 & 2.14 & 48.56 & 54.78 & 0.17 & 47.94 & 45.57 & 0.48 & 39.90 & 55.03 & 1.15 & 48.21 \\
 & \acd{} & 71.36 & 0.92 & 62.50 & 64.55 & 0.15 & 56.48 & 66.66 & 0.18 & 58.33 & 68.48 & 0.00 & 59.93 \\
 & \abstain{} & 60.22 & 52.05 & 48.17 & 38.73 & 45.16 & 26.73 & 50.49 & 46.62 & 37.83 & 61.86 & 53.29 & 52.85 \\
 & \sa{} & 57.23 & 48.11 & 43.91 & 56.81 & 10.95 & 50.17 & 59.37 & 20.80 & 52.98 & 62.52 & 49.03 & 57.49 \\
 & \ent{} & 64.06 & 53.34 & 55.53 & 58.00 & 41.09 & 51.98 & 59.23 & 42.61 & 52.75 & 61.91 & 56.29 & 55.48 \\
 & \fsb{} & 69.27 & 54.94 & 59.64 & 55.04 & 47.26 & 43.26 & 62.44 & \underline{47.60} & 53.66 & 66.71 & 55.51 & 58.95 \\
 & \acda{} & 63.56 & 52.46 & 53.99 & 48.82 & 39.52 & 37.55 & 57.96 & 46.34 & 49.28 & 61.46 & 54.02 & 55.80 \\
 \cmidrule(r){2-14}
 & \method{} & \underline{72.06} & \textbf{55.49} & \underline{62.95} & \underline{66.86} & \underline{47.52} & \underline{59.86} & \underline{68.62} & 47.14 & \underline{61.63} & \underline{69.68} & \underline{56.47} & \underline{61.45} \\
 & \methodm{} & \textbf{73.15} & \underline{55.47} & \textbf{63.72} & \textbf{69.99} & \textbf{47.60} & \textbf{62.28} & \textbf{70.66} & \textbf{48.12} & \textbf{63.18} & \textbf{71.00} & \textbf{56.46} & \textbf{62.30} \\ 
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \midrule
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multirow{10}{*}{HotpotQA} & 
\context{} & 57.15 & 1.19 & 50.08 & 57.14 & 0.00 & 49.98 & 57.16 & 0.10 & 50.00 & 56.99 & 0.09 & 49.88 \\
 & \cad{} & 55.78 & 1.88 & 48.89 & 54.68 & 0.04 & 47.84 & 54.60 & 0.07 & 47.76 & 53.74 & 0.20 & 47.04 \\
 & \acd{} & 74.36 & 0.57 & 65.09 & 69.27 & 0.00 & 60.60 & 69.80 & 0.07 & 61.15 & 72.72 & 0.09 & 63.64 \\
 & \abstain{} & 66.88 & 56.58 & 56.23 & 47.29 & \underline{48.65} & 33.49 & 57.17 & 51.95 & 43.02 & 61.12 & 54.66 & 53.06 \\
 & \sa{} & 50.64 & 48.63 & 33.86 & 58.58 & 17.35 & 52.19 & 58.22 & 14.36 & 51.87 & 61.33 & 43.36 & 56.36 \\
 & \ent{} & 67.08 & 56.44 & 57.92 & 59.00 & 45.11 & 52.64 & 59.24 & 45.47 & 53.01 & 63.31 & \textbf{60.07} & 57.19 \\
 & \fsb{} & 74.89 & 58.51 & 66.21 & 65.63 & \textbf{53.82} & 55.73 & 68.68 & 54.16 & 60.41 & 74.32 & 52.18 & 68.20 \\
 & \acda{} & 65.88 & 54.67 & 57.41 & 57.79 & 51.11 & 47.90 & 62.00 & 52.13 & 54.03 & 61.02 & 50.93 & 57.01 \\
 \cmidrule(r){2-14}
 & \method{} & \underline{78.71} & \underline{62.50} & \underline{70.20} & \underline{73.39} & 42.41 & \underline{66.96} & \textbf{73.69} & \underline{56.81} & \underline{68.98} & \underline{76.28} & 55.84 & \underline{69.43} \\
 & \methodm{} & \textbf{79.32} & \textbf{62.59} & \textbf{70.64} & \textbf{74.09} & 42.31 & \textbf{67.50} & \underline{73.66} & \textbf{56.89} & \textbf{68.92} & \textbf{76.94} & \underline{56.67} & \textbf{69.98} \\ 
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \midrule
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multirow{10}{*}{TriviaQA} & 
\context{} & 57.29 & 2.24 & 50.23 & 57.17 & 0.26 & 50.02 & 57.15 & 0.47 & 50.03 & 57.13 & 0.35 & 50.00 \\
 & \cad{} & 55.83 & 0.65 & 48.87 & 55.11 & 0.25 & 48.22 & 55.81 & 0.32 & 48.84 & 54.71 & 0.57 & 47.89 \\
 & \acd{} & 76.79 & 3.09 & 67.38 & 72.86 & 0.18 & 63.74 & \underline{72.49} & 0.42 & 63.43 & 75.01 & 0.05 & 65.62 \\
 & \abstain{} & 67.46 & 57.31 & 56.21 & 59.19 & 50.45 & 47.04 & 48.53 & 46.74 & 35.11 & 60.73 & 53.16 & 51.25 \\
 & \sa{} & 52.40 & 48.38 & 36.73 & 57.93 & 8.97 & 51.05 & 58.09 & 12.07 & 51.53 & 62.18 & 48.60 & 57.19 \\
 & \ent{} & 66.17 & 57.26 & 56.50 & 60.21 & 47.84 & 53.99 & 60.21 & 48.31 & 54.31 & 62.21 & \underline{56.59} & 56.23 \\
 & \fsb{} & 77.02 & 59.84 & 68.55 & 69.50 & \underline{51.88} & 60.41 & 66.21 & \underline{52.08} & 56.12 & 77.67 & 47.53 & \textbf{70.69} \\
 & \acda{} & 66.67 & 56.73 & 58.81 & 61.21 & 50.52 & 53.09 & 58.42 & 49.72 & 49.22 & 61.62 & 51.62 & 56.81 \\
\cmidrule(r){2-14}
 & \method{} & \underline{80.39} & \textbf{65.67} & \underline{72.35} & \textbf{73.70} & 51.29 & \textbf{67.29} & 71.08 & 51.44 & \underline{64.08} & \underline{75.76} & 56.35 & 67.57 \\
 & \methodm{} & \textbf{80.93} & \underline{65.66} & \textbf{72.74} & \underline{73.47} & \textbf{52.10} & \underline{67.11} & \textbf{73.12} & \textbf{53.46} & \textbf{65.82} & \textbf{76.95} & \textbf{57.06} & \underline{68.38} \\ 
 \bottomrule
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{tabular}



    
    }
    \caption{
        Experimental results on three different datasets.
        For each dataset, the \textbf{best method} is highlighted in bold, and the \underline{second-best method} is underlined.
        \method{} and \methodm{} outperform all the baselines across different metrics.
    }
    \label{table:main_results}
\end{table*}

==> assets/tables/main_results_v2.tex <==
\definecolor{my_gray}{HTML}{E8E8E8}
\newcolumntype{g}{>{\columncolor{my_gray}}c}

% \setlength{\aboverulesep}{0pt}
% \setlength{\belowrulesep}{0pt}
% \setlength{\extrarowheight}{.75ex}


\begin{table*}[t!]
    \centering    
    \resizebox{0.91\textwidth}{!}{

    
% \begin{tabular}{cccccccccccccccc}
\begin{tabular}{cgggggcccccggggg}
\toprule
\multirow{2}{*}{Method} & 
\multicolumn{5}{c}{NQ} & 
\multicolumn{5}{c}{HotpotQA} & 
\multicolumn{5}{c}{TriviaQA} \\
\cmidrule(l){2-6} \cmidrule(l){7-11} \cmidrule(l){12-16} 
\rowcolor{white}
 & F1$_{\text{ans}}$ & F1$_{\text{abs}}$ & RS & Acc. & Cov. & 
 F1$_{\text{ans}}$ & F1$_{\text{abs}}$ & RS & Acc. & Cov. & 
 F1$_{\text{ans}}$ & F1$_{\text{abs}}$ & RS & Acc. & Cov. \\ 
 \midrule
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multicolumn{16}{l}{\textbf{\ml{}}} \\ 
\midrule
context & 57.26 & 2.18 & 50.22 & 49.95 & 50.23 & 57.15 & 1.19 & 50.08 & 49.93 & 50.08 & 57.29 & 2.24 & 50.23 & 49.95 & 50.23 \\
cad & 60.22 & 52.05 & 48.17 & 38.36 & 57.27 & 66.88 & 56.58 & 56.23 & 45.21 & 63.55 & 67.46 & 57.31 & 56.21 & 45.07 & 64.10 \\
acd & 55.34 & 2.14 & 48.56 & 48.29 & 48.56 & 55.78 & 1.88 & 48.89 & 51.99 & 48.89 & 55.83 & 0.65 & 48.87 & 48.79 & 48.87 \\
abstain & 71.36 & 0.92 & 62.50 & \textbf{62.39} & 62.50 & 74.36 & 0.57 & 65.09 & \textbf{65.02} & 65.09 & 76.79 & 3.09 & 67.38 & \textbf{66.99} & 67.39 \\
sa & 57.23 & 48.11 & 43.91 & 35.06 & 53.70 & 50.64 & 48.63 & 33.86 & 26.80 & 49.70 & 52.40 & 48.38 & 36.73 & 29.01 & 50.61 \\
fsb & 69.27 & 54.94 & 59.64 & 49.02 & 65.09 & 74.89 & 58.51 & 66.21 & 55.05 & 70.55 & 77.02 & 59.84 & 68.55 & 57.24 & 72.62 \\
acda & 63.56 & 52.46 & 53.99 & 43.82 & 60.11 & 65.88 & 54.67 & 57.41 & 46.80 & 62.63 & 66.67 & 56.73 & 58.81 & 57.88 & 63.87 \\
method & 72.06 & \textbf{54.49} & 62.95 & 52.28 & 67.51 & 78.71 & 62.50 & 70.20 & 58.36 & 74.52 & 80.39 & \textbf{65.67} & 72.35 & 60.01 & 76.67 \\
methodm & \textbf{73.15} & 55.47 & \textbf{63.72} & 53.16 & \textbf{68.30} & \textbf{79.32} & \textbf{62.59} & \textbf{70.64} & 58.78 & \textbf{74.99} & \textbf{80.93} & 65.66 & \textbf{72.74} & 60.40 & \textbf{77.07} \\
\midrule
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multicolumn{16}{l}{\textbf{\mll{}}} \\ 
\midrule
context & 57.13 & 0.09 & 49.98 & 49.97 & 49.98 & 57.14 & 0.00 & 49.98 & 49.98 & 49.98 & 57.17 & 0.26 & 50.02 & 49.99 & 50.02 \\
cad & 38.73 & 45.16 & 26.73 & 20.54 & 42.11 & 47.29 & 48.65 & 33.49 & 26.18 & 48.18 & 59.19 & 50.45 & 47.04 & 37.87 & 56.27 \\
acd & 54.78 & 0.17 & 47.94 & 47.92 & 47.94 & 54.68 & 0.04 & 47.84 & 47.84 & 47.84 & 55.11 & 0.25 & 48.22 & 48.19 & 48.22 \\
abstain & 64.55 & 0.15 & 56.48 & \textbf{56.46} & 56.48 & 69.27 & 0.00 & 60.60 & 60.60 & 60.60 & 72.86 & 0.18 & 63.74 & \textbf{63.72} & 63.74 \\
sa & 56.81 & 10.95 & 50.17 & 48.66 & 50.23 & 58.58 & 17.35 & 52.19 & 49.70 & 52.33 & 57.93 & 8.97 & 51.05 & 49.84 & 51.09 \\
fsb & 55.04 & \textbf{47.26} & 43.26 & 34.47 & 52.20 & 65.63 & \textbf{53.82} & 55.73 & 45.37 & 62.04 & 69.50 & \textbf{51.88} & 60.41 & 50.59 & 64.78 \\
acda & 48.82 & 39.52 & 37.55 & 30.41 & 45.66 & 57.79 & 51.11 & 47.90 & 38.19 & 55.61 & 61.21 & 50.52 & 53.09 & 43.46 & 58.18 \\
method & 66.66 & 45.63 & 59.49 & 51.22 & 61.90 & 73.39 & 42.41 & 66.96 & 60.15 & 67.82 & 73.14 & 48.86 & 66.59 & 58.19 & 68.22 \\
methodm & \textbf{69.78} & 45.71 & \textbf{61.91} & 53.62 & \textbf{64.33} & \textbf{74.09} & 42.31 & \textbf{67.50} & \textbf{60.70} & \textbf{68.37} & \textbf{73.70} & 49.97 & \textbf{67.15} & 58.53 & \textbf{68.88} \\
\midrule
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multicolumn{16}{l}{\textbf{\mlll{}}} \\ 
\midrule
context & 57.14 & 0.37 & 50.00 & 49.95 & 50.00 & 57.16 & 0.10 & 50.00 & 49.98 & 50.00 & 57.15 & 0.47 & 50.03 & 49.97 & 50.03 \\
cad & 50.49 & 46.62 & 37.83 & 29.70 & 48.93 & 57.17 & 51.95 & 43.02 & 33.89 & 55.10 & 48.53 & 46.74 & 35.11 & 27.52 & 47.88 \\
acd & 45.57 & 0.48 & 39.90 & 39.84 & 39.90 & 54.60 & 0.07 & 47.76 & 47.75 & 47.76 & 55.81 & 0.32 & 48.84 & 48.80 & 48.84 \\
abstain & 66.66 & 0.18 & 58.33 & \textbf{58.31} & 58.33 & 69.80 & 0.07 & 61.15 & \textbf{61.14} & 61.15 & 72.49 & 0.42 & 63.43 & \textbf{63.38} & 63.43 \\
sa & 59.37 & 20.80 & 52.98 & 49.89 & 53.21 & 58.22 & 14.36 & 51.87 & 49.89 & 51.95 & 58.09 & 12.07 & 51.53 & 49.85 & 51.59 \\
fsb & 62.44 & \textbf{47.60} & 53.66 & 44.46 & 58.19 & 68.68 & 54.16 & 60.41 & 50.05 & 64.79 & 66.21 & \textbf{52.08} & 56.12 & 45.98 & 61.91 \\
acda & 57.96 & 46.34 & 49.28 & 40.27 & 54.43 & 62.00 & 52.13 & 54.03 & 43.95 & 59.16 & 58.42 & 49.72 & 49.22 & 39.54 & 55.61 \\
method & 68.32 & 44.63 & 61.14 & 53.16 & 63.08 & \textbf{73.69} & 56.81 & \textbf{68.98} & 59.53 & \textbf{70.44} & 70.71 & 48.37 & 63.47 & 54.78 & 65.72 \\
methodm & \textbf{70.35} & 45.73 & \textbf{62.70} & 54.46 & \textbf{64.81} & 73.66 & \textbf{56.89} & 68.92 & 59.42 & 70.42 & \textbf{72.74} & 50.49 & \textbf{65.22} & 56.09 & \textbf{67.68} \\
\midrule
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multicolumn{16}{l}{\textbf{\mm{}}} \\ 
\midrule
context & 57.04 & 0.25 & 49.88 & 49.85 & 49.88 & 56.99 & 0.09 & 49.88 & 49.87 & 49.88 & 57.13 & 0.35 & 50.00 & 49.96 & 50.00 \\
cad & 61.86 & 53.29 & 52.85 & 42.83 & 59.70 & 61.12 & 54.66 & 53.06 & 42.55 & 59.23 & 60.73 & 53.16 & 51.25 & 41.22 & 58.42 \\
acd & 55.03 & 1.15 & 48.21 & 48.07 & 48.21 & 53.74 & 0.20 & 47.04 & 47.01 & 47.04 & 54.71 & 0.57 & 47.89 & 47.82 & 47.89 \\
abstain & 68.48 & 0.00 & 59.93 & \textbf{59.93} & 59.93 & 72.72 & 0.09 & 63.64 & \textbf{63.62} & 63.64 & 75.01 & 0.05 & 65.62 & \textbf{65.62} & 65.62 \\
sa & 62.52 & 49.03 & 57.49 & 48.76 & 59.54 & 61.33 & 43.36 & 56.36 & 48.95 & 57.70 & 62.18 & 48.60 & 57.19 & 48.55 & 59.20 \\
fsb & 66.71 & 55.51 & 58.95 & 48.32 & 63.65 & 74.32 & 52.18 & 68.20 & 59.27 & 69.94 & 77.67 & 47.53 & \textbf{70.69} & 62.72 & 72.07 \\
acda & 61.46 & 54.02 & 55.80 & 45.58 & 59.56 & 61.02 & 50.93 & 57.01 & 48.10 & 58.95 & 61.62 & 51.62 & 56.81 & 47.48 & 59.48 \\
method & 69.68 & 56.47 & 61.45 & 50.61 & 66.09 & 76.28 & 55.84 & 69.43 & 59.50 & 71.83 & 75.76 & 56.35 & 67.57 & 57.21 & 71.21 \\
methodm & \textbf{71.00} & \textbf{56.46} & \textbf{62.30} & 51.45 & \textbf{67.03} & \textbf{76.94} & \textbf{56.67} & \textbf{69.98} & 59.85 & \textbf{72.49} & \textbf{76.95} & \textbf{57.06} & 68.38 & 57.84 & \textbf{72.21} \\
\bottomrule
\end{tabular}



    
    }
    \caption{
        Experimental results on three different datasets.
        For each dataset, the \textbf{best method} is highlighted in bold, and the \underline{second-best method} is underlined.
        \method{} and \methodm{} outperform all the baselines across different metrics.
    }
    \label{table:main_results_v2}
\end{table*}

==> assets/tables/main_results_v3.tex <==
\definecolor{my_gray}{HTML}{E8E8E8}
\newcolumntype{g}{>{\columncolor{my_gray}}c}



\begin{table*}[t!]
    \centering    
    \resizebox{0.9\textwidth}{!}{

  \begin{tabular}{cgggcccgggccc}
\toprule

Backbone &
\multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}} {\scshape Llama3 8B}\\ {\scshape Instruct}\end{tabular}} &
\multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}} {\scshape Llama2 7B}\\ {\scshape Chat}\end{tabular}} &
\multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}} {\scshape Llama2 13B}\\ {\scshape Chat}\end{tabular}} &
\multicolumn{3}{c}{\begin{tabular}[c]{@{}c@{}} {\scshape Mistral 7B}\\ {\scshape Instruct}\end{tabular}} \\
\midrule
% \cmidrule(l){1-2} \cmidrule(l){3-5} \cmidrule(l){6-8} \cmidrule(l){9-11} \cmidrule(l){12-14} 
Method & \multicolumn{1}{c}{\abs{}} & \multicolumn{1}{c}{\ans{}} & \multicolumn{1}{c}{RS} &
\multicolumn{1}{c}{\abs{}} & \multicolumn{1}{c}{\ans{}} & \multicolumn{1}{c}{RS} &
\multicolumn{1}{c}{\abs{}} & \multicolumn{1}{c}{\ans{}} & \multicolumn{1}{c}{RS} &
\multicolumn{1}{c}{\abs{}} & \multicolumn{1}{c}{\ans{}} & \multicolumn{1}{c}{RS} \\ 
\midrule
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multicolumn{13}{c}{NQ} \\
\midrule
\context{} & 57.26 & 2.18 & 50.22 & 57.13 & 0.09 & 49.98 & 57.14 & 0.37 & 50.00 & 57.04 & 0.25 & 49.88 \\
 \cad{} & 60.22 & 52.05 & 48.17 & 38.73 & 45.16 & 26.73 & 50.49 & 46.62 & 37.83 & 61.86 & 53.29 & 52.85 \\
 \acd{} & 55.34 & 2.14 & 48.56 & 54.78 & 0.17 & 47.94 & 45.57 & 0.48 & 39.90 & 55.03 & 1.15 & 48.21 \\
 \abstain{} & 71.36 & 0.92 & 62.50 & 64.55 & 0.15 & 56.48 & 66.66 & 0.18 & 58.33 & 68.48 & 0.00 & 59.93 \\
 \sa{} & 57.23 & 48.11 & 43.91 & 56.81 & 10.95 & 50.17 & 59.37 & 20.80 & 52.98 & 62.52 & 49.03 & 57.49 \\
 \fsb{} & 69.27 & 54.94 & 59.64 & 55.04 & 47.26 & 43.26 & 62.44 & \underline{47.60} & 53.66 & 66.71 & 55.51 & 58.95 \\
 \acda{} & 63.56 & 52.46 & 53.99 & 48.82 & 39.52 & 37.55 & 57.96 & 46.34 & 49.28 & 61.46 & 54.02 & 55.80 \\
\midrule
\method{} & \underline{72.06} & \textbf{55.49} & \underline{62.95} & \underline{66.86} & \underline{47.52} & \underline{59.86} & \underline{68.62} & 47.14 & \underline{61.63} & \underline{69.68} & \underline{56.47} & \underline{61.45} \\
 \methodm{} & \textbf{73.15} & \underline{55.47} & \textbf{63.72} & \textbf{69.99} & \textbf{47.60} & \textbf{62.28} & \textbf{70.66} & \textbf{48.12} & \textbf{63.18} & \textbf{71.00} & \textbf{56.46} & \textbf{62.30} \\ 
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \midrule
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multicolumn{13}{c}{HotpotQA} \\
\midrule
\context{} & 57.15 & 1.19 & 50.08 & 57.14 & 0.00 & 49.98 & 57.16 & 0.10 & 50.00 & 56.99 & 0.09 & 49.88 \\
 \cad{} & 66.88 & 56.58 & 56.23 & 47.29 & \underline{48.65} & 33.49 & 57.17 & 51.95 & 43.02 & 61.12 & 54.66 & 53.06 \\
 \acd{} & 55.78 & 1.88 & 48.89 & 54.68 & 0.04 & 47.84 & 54.60 & 0.07 & 47.76 & 53.74 & 0.20 & 47.04 \\
 \abstain{} & 74.36 & 0.57 & 65.09 & 69.27 & 0.00 & 60.60 & 69.80 & 0.07 & 61.15 & 72.72 & 0.09 & 63.64 \\
 \sa{} & 50.64 & 48.63 & 33.86 & 58.58 & 17.35 & 52.19 & 58.22 & 14.36 & 51.87 & 61.33 & 43.36 & 56.36 \\
 \fsb{} & 74.89 & 58.51 & 66.21 & 65.63 & \textbf{53.82} & 55.73 & 68.68 & 54.16 & 60.41 & 74.32 & 52.18 & 68.20 \\
 \acda{} & 65.88 & 54.67 & 57.41 & 57.79 & 51.11 & 47.90 & 62.00 & 52.13 & 54.03 & 61.02 & 50.93 & 57.01 \\
 \midrule
 \method{} & \underline{78.71} & \underline{62.50} & \underline{70.20} & \underline{73.39} & 42.41 & \underline{66.96} & \textbf{73.69} & \underline{56.81} & \underline{68.98} & \underline{76.28} & \underline{55.84} & \underline{69.43} \\
 \methodm{} & \textbf{79.32} & \textbf{62.59} & \textbf{70.64} & \textbf{74.09} & 42.31 & \textbf{67.50} & \underline{73.66} & \textbf{56.89} & \textbf{68.92} & \textbf{76.94} & \textbf{56.67} & \textbf{69.98} \\ 
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \midrule
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\multicolumn{13}{c}{TriviaQA} \\
\midrule
\context{} & 57.29 & 2.24 & 50.23 & 57.17 & 0.26 & 50.02 & 57.15 & 0.47 & 50.03 & 57.13 & 0.35 & 50.00 \\
 \cad{} & 67.46 & 57.31 & 56.21 & 59.19 & 50.45 & 47.04 & 48.53 & 46.74 & 35.11 & 60.73 & 53.16 & 51.25 \\
 \acd{} & 55.83 & 0.65 & 48.87 & 55.11 & 0.25 & 48.22 & 55.81 & 0.32 & 48.84 & 54.71 & 0.57 & 47.89 \\
 \abstain{} & 76.79 & 3.09 & 67.38 & 72.86 & 0.18 & 63.74 & \underline{72.49} & 0.42 & 63.43 & 75.01 & 0.05 & 65.62 \\
 \sa{} & 52.40 & 48.38 & 36.73 & 57.93 & 8.97 & 51.05 & 58.09 & 12.07 & 51.53 & 62.18 & 48.60 & 57.19 \\
 \fsb{} & 77.02 & 59.84 & 68.55 & 69.50 & \underline{51.88} & 60.41 & 66.21 & \underline{52.08} & 56.12 & 77.67 & 47.53 & \textbf{70.69} \\
 \acda{} & 66.67 & 56.73 & 58.81 & 61.21 & 50.52 & 53.09 & 58.42 & 49.72 & 49.22 & 61.62 & 51.62 & 56.81 \\
\midrule
\method{} & \underline{80.39} & \textbf{65.67} & \underline{72.35} & \textbf{73.70} & 51.29 & \textbf{67.29} & 71.08 & 51.44 & \underline{64.08} & \underline{75.76} & \underline{56.35} & 67.57 \\
 \methodm{} & \textbf{80.93} & \underline{65.66} & \textbf{72.74} & \underline{73.47} & \textbf{52.10} & \underline{67.11} & \textbf{73.12} & \textbf{53.46} & \textbf{65.82} & \textbf{76.95} & \textbf{57.06} & \underline{68.38} \\ 
 \bottomrule
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{tabular}



    
    }
    \caption{
        Experimental results on three different datasets.
        For each dataset, the \textbf{best method} is highlighted in bold, and the \underline{second-best method} is underlined.
        \method{} and \methodm{} outperform all the baselines across different metrics.
    }
    \label{table:main_results_v3}
\end{table*}

==> assets/tables/rag.tex <==

\begin{table}[t]
    \centering    
    % \small
    \resizebox{0.65\linewidth}{!}{

% \begin{tabular}{ccccc}
% \toprule
% Method & NQ & HotpotQA & TriviaQA & Avg. \\ 
% \midrule
% \abstain{} & 40.86 & 34.32 & 66.87 & 44.56 \\
% \sa{} & 37.72 & 36.52 & 65.93 & 43.97 \\
% \fsb{} & \underline{47.49} & 45.81 & 73.83 & 52.43 \\
% \acda{} & 45.52 & 43.54 & 70.58 & 50.08 \\ 
% \midrule
% \method{} & \textbf{50.55} & \underline{46.96} & \underline{76.14} & \underline{54.48} \\
% \methodm{} & \textbf{50.55} & \textbf{47.17} & \textbf{76.63} & \textbf{54.70} \\ 
% \bottomrule
% \end{tabular}

\begin{tabular}{ccccc}
\toprule
Method & NQ & HotpotQA & TriviaQA \\ 
\midrule
\abstain{} & 40.86 & 34.32 & 66.87 \\
\sa{} & 37.72 & 36.52 & 65.93 \\
\fsb{} & \underline{47.49} & 45.81 & 73.83 \\
\acda{} & 45.52 & 43.54 & 70.58 \\ 
\midrule
\method{} & \textbf{50.55} & \underline{46.96} & \underline{76.14} \\
\methodm{} & \textbf{50.55} & \textbf{47.17} & \textbf{76.63} \\ 
\bottomrule
\end{tabular}

    
    }
    \caption{
        Average Reliability Score (RS) in RAG settings.
        The \textbf{best method} is in bold, and the \underline{second-best method} is underlined.
        \method{}({\scshape -m}) outperform all the baselines.
        % \method{} and \methodm{} outperform all the baselines.
        % Full results are presented in Table \ref{table:rag_full}.
    }
    \label{table:rag_results}
\end{table}




==> assets/tables/trained_methods_2.tex <==
\definecolor{bg}{HTML}{b1d4e0}

\begin{table}[t]
    \centering
        
    \begin{subfigure}{0.99\columnwidth}
        
        \resizebox{\linewidth}{!}{

        \begin{tabular}{cccccccccc}
        \toprule
        Target ($\rightarrow$) & \multicolumn{3}{c}{NQ} & \multicolumn{3}{c}{HotpotQA} & \multicolumn{3}{c}{TriviaQA} \\ 
        \midrule
        Source ($\downarrow$) & \ans{} & \abs{} & RS & \ans{} & \abs{} & RS & \ans{} & \abs{} & RS \\ 
        \midrule
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        NQ & 
        \cellcolor{bg}\underline{64.86} & \cellcolor{bg}\underline{46.56} & \cellcolor{bg}\underline{58.03} & 
        66.62 & 52.36 & 58.50 & 
        65.07 & \underline{53.52} & 57.39 \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        HotpotQA & 
        61.46 & 38.42 & 54.60 & 
        \cellcolor{bg}\underline{68.41} & \cellcolor{bg}\underline{56.92} & \cellcolor{bg}\underline{60.80} & 
        60.09 & 38.53 & 53.28 \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        TriviaQA & 
        63.30 & 45.10 & 55.55 & 
        66.97 & 54.88 & 59.24 & 
        \cellcolor{bg}\underline{65.31} & \cellcolor{bg}52.63 & \cellcolor{bg}\underline{58.13} \\ 
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \midrule
        \methodm{} & 
        \textbf{73.15} & \textbf{55.47} & \textbf{63.72} & 
        \textbf{79.32} & \textbf{62.59} & \textbf{70.64} & 
        \textbf{80.93} & \textbf{65.66} & \textbf{72.74} \\ 
        \bottomrule
        \end{tabular}

        }
         
        \caption{Results of external verifier.}
        
    \end{subfigure}

    \begin{subfigure}{0.99\columnwidth}
        \resizebox{\linewidth}{!}{

        \begin{tabular}{cccccccccc}
        \toprule
        Target ($\rightarrow$) & \multicolumn{3}{c}{NQ} & \multicolumn{3}{c}{HotpotQA} & \multicolumn{3}{c}{TriviaQA} \\ 
        \midrule
        Source ($\downarrow$) & \ans{} & \abs{} & RS & \ans{} & \abs{} & RS & \ans{} & \abs{} & RS \\ 
        \midrule
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        NQ & 
        \cellcolor{bg}\underline{66.37} & \cellcolor{bg}43.87 & \cellcolor{bg}\underline{61.12} & 
        64.43 & 48.79 & 59.65 & 
        67.31 & 49.00 & \underline{62.14} \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        HotpotQA & 
        64.86 & 42.73 & 59.80 & 
        \cellcolor{bg}\underline{74.06} & \cellcolor{bg}\underline{57.57} & \cellcolor{bg}\underline{68.76} & 
        65.26 & 50.69 & 61.17 \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        TriviaQA & 
        65.15 & \underline{46.37} & 57.70 & 
        66.68 & 49.82 & 60.58 & 
        \cellcolor{bg}\underline{67.60} & \cellcolor{bg}\underline{53.68} & \cellcolor{bg}61.84 \\ 
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \midrule
        \methodm{} & 
        \textbf{73.15} & \textbf{55.47} & \textbf{63.72} & 
        \textbf{79.32} & \textbf{62.59} & \textbf{70.64} & 
        \textbf{80.93} & \textbf{65.66} & \textbf{72.74} \\ 
        \bottomrule
        \end{tabular}
        
        }
        \caption{Results of instruction-tuning.}
        
    \end{subfigure}
    
    \caption{
        % The results of the trained methods and \methodm{}.
        The results compared to training-based methods.
        \colorbox{bg}{In-domain} results are highlighted in blue, the \textbf{best results} are in bold, and the \underline{second-based results} are underlined.
        \methodm{} outperforms the training-based methods across all the scenarios.
    }
    \label{table:trained_methods}
\end{table}


==> assets/templates/abstain.tex <==

\begin{table}[t]
    \centering    

    \small
    \ttfamily
    \begin{tabularx}{\linewidth}{X}
    \toprule  
Answer the following question based on the given context. If you are unsure or don't know the correct answer, simply respond with "Unknown." \\\\

\textcolor{brown}{<few-shot demonstrations>} \\\\

Context: \textcolor{brown}{<context>} \\
Question: \textcolor{brown}{<question>} \\
Answer: 
\\
    \bottomrule
\end{tabularx}

    \caption{
        Template with explicit instruction for abstention
        % Template with an explicit instruction for abstention.
    }
    % \label{template:abstain}
\end{table}

==> assets/templates/contextual.tex <==

\begin{table}[t]
    \centering    

    \footnotesize
    \ttfamily
    \begin{tabularx}{\linewidth}{X}
    \toprule
    

Answer the following question based on the given context. \\\\

\textcolor{brown}{<few-shot demonstrations>} \\\\

Context: \textcolor{brown}{<context>} \\
Question: \textcolor{brown}{<question>} \\
Answer: 
\\

    \bottomrule
\end{tabularx}

    \caption{
        % Inference template $\text{T}_c(\cdot)$ employing contextual knowledge.
        Template employing contextual knowledge.
    }
    % \label{template:context}
\end{table}

==> assets/templates/parametric.tex <==

\begin{table}[t]
    \centering    

    \footnotesize
    \ttfamily
    \begin{tabularx}{\linewidth}{X}
    \toprule
Answer the following question. \\\\

\textcolor{brown}{<few-shot demonstrations>} \\\\

Question: \textcolor{brown}{<question>} \\
Answer: 
\\
    \bottomrule
    \end{tabularx}

    \caption{
        % Template $\text{T}_p(\cdot)$ for utilizing parametric knowledge.
        Template utilizing parametric knowledge.
    }
    % \label{template:param}
\end{table}
